Short reasons for long vectors in HPC CPUs: a study based on RISC-V

For years, SIMD/vector units have enhanced the capabilities of modern CPUs in High-Performance Computing (HPC) and mobile technology. Typical commercially-available SIMD units process up to 8 double-precision elements with one instruction. The optimal vector width and its impact on CPU throughput due to memory latency and bandwidth remain challenging research areas. This study examines the behavior of four computational kernels on a RISC-V core connected to a customizable vector unit, capable of operating up to 256 double precision elements per instruction. The four codes have been purposefully selected to represent non-dense workloads: SpMV, BFS, PageRank, FFT. The experimental setup allows us to measure their performance while varying the vector length, the memory latency, and bandwidth. Our results not only show that larger vector lengths allow for better tolerance of limitations in the memory subsystem but also offer hope to code developers beyond dense linear algebra.

==> 90-acks.tex <==
%%
%% The acknowledgments section is defined using the "acks" environment
%% (and NOT an unnumbered section). This ensures the proper
%% identification of the section in the article metadata, and the
%% consistent spelling of the heading.
\begin{acks}
This research received funding from the EU-HPC-JU under FPA N.~800928 (EPI) and SGA N.~101036168 (EPI-SGA2). The JU receives support from some member countries. The EPI-SGA2 project, PCI2022-132935 is also co-funded by MCIN/AEI /10.13039/501100011033 and by the UE NextGenerationEU/PRTR.
\end{acks}



==> makefile <==
MAIN=short-reasons-for-long-vectors
PDF_VIEWER=/usr/bin/atril
ENGINE=pdflatex

all: full

full: clean
	$(ENGINE) $(MAIN).tex
	bibtex $(MAIN)
	$(ENGINE) $(MAIN).tex
	$(ENGINE) $(MAIN).tex

diff: clean
	scratch/my_diff.sh ; \
	$(ENGINE) $(MAIN).tex && \
	bibtex $(MAIN) && \
	$(ENGINE) $(MAIN).tex && \
	$(ENGINE) $(MAIN).tex && \
	mv $(MAIN).pdf $(MAIN)_DIFF.pdf && \
	git checkout .

view:
	$(PDF_VIEWER) $(MAIN).pdf

revision: full
	cp $(MAIN).pdf $(MAIN)-$(shell git rev-parse --short HEAD).pdf

clean:
	rm -fv $(MAIN).acn $(MAIN).acr $(MAIN).alg $(MAIN).aux $(MAIN).glg $(MAIN).glo $(MAIN).gls $(MAIN).ist $(MAIN).log $(MAIN).out $(MAIN).pdf $(MAIN).toc  $(MAIN).blg $(MAIN).brf $(MAIN).lof missfont.log $(MAIN).fls $(MAIN).fdb_latexmk $(MAIN).spl


